The Transformation of Broadband Demand: From Discretionary Service to Essential Infrastructure (2010-2024)

Has broadband become a necessity good immune to price changes? Using a 15-year panel of 33 European countries (2010--2024) and two-way fixed effects with Driscoll--Kraay standard errors, we document a fundamental transformation in broadband demand. Pre-COVID, Eastern Partnership countries exhibited highly elastic demand ($\varepsilon = -0.61$, p$<$0.001) -- a 10\% price reduction increased subscriptions by 6\% -- while EU countries showed moderate elasticity ($\varepsilon = -0.12$, p$<$0.05). By 2020--2024, both regions converged to near-zero elasticity, with price changes having no detectable effect on adoption. Crucially, placebo tests reveal this transformation began in 2015, not 2020, indicating a decade-long digital integration process rather than a COVID-19 shock. We further demonstrate that price measurement critically affects inference: income-relative prices (as \% of GNI) yield significant results in 100\% of specifications, compared to only 25\% for PPP-adjusted prices. These findings have immediate policy relevance: as broadband transitions from discretionary service to essential utility, policy emphasis must shift from affordability subsidies to universal infrastructure deployment.

==> table1_baseline_copy.tex <==
\begin{table}[p]
\centering
\caption{Baseline Two-Way Fixed Effects Estimates: Pre-COVID Period (2010--2019)}
\label{tab:baseline}
\begin{threeparttable}
\begin{adjustbox}{width=\textwidth}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{@{}lccccccc@{}}
\toprule
& \multicolumn{7}{c}{Dependent Variable: Log(Subscriptions per 100)} \\
\cmidrule(lr){2-8}
& (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
& GDP Only & + Socio & + Instit. & + Infra. & + Demog. & + All & Full \\
\midrule
\textbf{Panel A: Price Elasticity} \\
Log(Price) & $-0.09^{*}$ & $-0.10^{**}$ & $-0.11^{**}$ & $-0.12^{**}$ & $-0.11^{**}$ & $-0.12^{**}$ & $-0.12^{**}$ \\
& (0.04) & (0.04) & (0.04) & (0.05) & (0.04) & (0.05) & (0.05) \\
\\
Log(Price) $\times$ EaP & $-0.47^{***}$ & $-0.48^{***}$ & $-0.49^{***}$ & $-0.50^{***}$ & $-0.48^{***}$ & $-0.49^{***}$ & $-0.49^{***}$ \\
& (0.09) & (0.09) & (0.09) & (0.09) & (0.09) & (0.09) & (0.09) \\
\\
\textit{Implied EaP elasticity} & $-0.56^{***}$ & $-0.58^{***}$ & $-0.60^{***}$ & $-0.62^{***}$ & $-0.59^{***}$ & $-0.61^{***}$ & $-0.61^{***}$ \\
& (0.08) & (0.08) & (0.08) & (0.08) & (0.08) & (0.08) & (0.08) \\
\midrule
\textbf{Panel B: Control Variables} \\
Log(GDP per capita) & $0.38^{***}$ & $0.40^{***}$ & $0.41^{***}$ & $0.42^{***}$ & $0.40^{***}$ & $0.42^{***}$ & $0.42^{***}$ \\
& (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) \\
\\
Urban population (\%) & & $0.012^{**}$ & $0.011^{**}$ & $0.010^{*}$ & $0.011^{**}$ & $0.010^{*}$ & $0.010^{*}$ \\
& & (0.005) & (0.005) & (0.005) & (0.005) & (0.005) & (0.005) \\
\\
Tertiary enrollment (\%) & & $0.008^{**}$ & $0.007^{*}$ & $0.007^{*}$ & $0.008^{**}$ & $0.007^{*}$ & $0.007^{*}$ \\
& & (0.003) & (0.003) & (0.003) & (0.003) & (0.003) & (0.003) \\
\\
Regulatory quality & & & $0.15^{*}$ & $0.14^{*}$ & $0.15^{*}$ & $0.14^{*}$ & $0.14^{*}$ \\
& & & (0.07) & (0.07) & (0.07) & (0.07) & (0.07) \\
\\
Log(Secure servers) & & & & $0.08^{**}$ & $0.09^{**}$ & $0.08^{**}$ & $0.08^{**}$ \\
& & & & (0.03) & (0.03) & (0.03) & (0.03) \\
\\
R\&D (\% GDP) & & & & $0.09^{*}$ & $0.10^{*}$ & $0.09^{*}$ & $0.09^{*}$ \\
& & & & (0.04) & (0.04) & (0.04) & (0.04) \\
\\
Log(Population density) & & & & & $0.06$ & $0.07$ & $0.07$ \\
& & & & & (0.08) & (0.08) & (0.08) \\
\\
Age dependency ratio & & & & & $-0.003$ & $-0.004$ & $-0.004$ \\
& & & & & (0.004) & (0.004) & (0.004) \\
\midrule
\textbf{Panel C: Model Statistics} \\
Country fixed effects & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
Year fixed effects & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
Observations & 297 & 297 & 297 & 297 & 297 & 297 & 297 \\
Countries & 33 & 33 & 33 & 33 & 33 & 33 & 33 \\
R-squared & 0.89 & 0.90 & 0.91 & 0.91 & 0.91 & 0.92 & 0.92 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\begin{tablenotes}[flushleft]
\scriptsize
\item \textit{Notes:} Dependent variable is log of fixed broadband subscriptions per 100 inhabitants. 
Price is measured as percentage of GNI per capita. EaP is a dummy for Eastern Partnership countries 
(Armenia, Azerbaijan, Belarus, Georgia, Moldova, Ukraine). All specifications include country and year 
fixed effects. Driscoll--Kraay standard errors (bandwidth = 3) in parentheses. 
$^{*}$ p $<$ 0.10, $^{**}$ p $<$ 0.05, $^{***}$ p $<$ 0.01.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> table2_covid_copy.tex <==
\begin{table}[p]
\centering
\caption{COVID-19 Interaction Effects: Full Sample (2010--2024)}
\label{tab:covid}
\begin{threeparttable}
\begin{adjustbox}{width=\textwidth}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{@{}lcccc@{}}
\toprule
& \multicolumn{4}{c}{Dependent Variable: Log(Subs. per 100)} \\
\cmidrule(lr){2-5}
& (1) & (2) & (3) & (4) \\
& Full Sample & Pre-COVID & COVID & Diff. Test \\
& w/ COVID Int. & 2010--19 & 2020--24 & (p-value) \\
\midrule
\textbf{Panel A: EU Countries} \\
Log(Price) & $-0.12^{**}$ & $-0.12^{**}$ & $+0.08$ & -- \\
& (0.05) & (0.05) & (0.09) & \\
\\
Log(Price) $\times$ COVID & $+0.31^{***}$ & -- & -- & 0.003 \\
& (0.10) & & & \\
\\
\textit{Implied COVID elasticity} & $+0.19$ & -- & $+0.08$ & -- \\
& (0.11) & & (0.09) & \\
\midrule
\textbf{Panel B: EaP Countries} \\
Log(Price) $\times$ EaP & $-0.49^{***}$ & $-0.49^{***}$ & $-0.11$ & -- \\
& (0.09) & (0.09) & (0.13) & \\
\\
Log(Price) $\times$ EaP $\times$ COVID & $+0.42^{***}$ & -- & -- & 0.001 \\
& (0.12) & & & \\
\\
\textit{Implied pre-COVID EaP elasticity} & $-0.61^{***}$ & $-0.61^{***}$ & -- & -- \\
& (0.08) & (0.08) & & \\
\\
\textit{Implied COVID EaP elasticity} & $-0.03$ & -- & $-0.03$ & -- \\
& (0.14) & & (0.13) & \\
\midrule
\textbf{Panel C: Change in Elasticity} \\
$\Delta\varepsilon_{EU}$ (COVID - Pre) & $+0.31^{***}$ & -- & -- & 0.003 \\
& (0.10) & & & \\
$\Delta\varepsilon_{EaP}$ (COVID - Pre) & $+0.58^{***}$ & -- & -- & $<$0.001 \\
& (0.11) & & & \\
\midrule
\textbf{Panel D: Model Statistics} \\
Full controls & Yes & Yes & Yes & -- \\
Country FE & Yes & Yes & Yes & -- \\
Year FE & Yes & Yes & Yes & -- \\
Observations & 495 & 297 & 198 & -- \\
Countries & 33 & 33 & 33 & -- \\
R-squared & 0.93 & 0.92 & 0.95 & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}
\begin{tablenotes}[flushleft]
\scriptsize
\begin{minipage}{\textwidth}
\item \textit{Notes:} Dependent variable is log of fixed broadband subscriptions per 100 inhabitants. 
Price is measured as percentage of GNI per capita. COVID is a period dummy for years 2020--2024. 
EaP is a dummy for Eastern Partnership countries. Full controls include: log GDP per capita, 
urban population \%, tertiary enrollment \%, regulatory quality, log secure servers, R\&D \% GDP, 
log population density, and age dependency ratio. Column (1) presents the full interaction model 
on 2010--2024 data. Columns (2)--(3) present separate subsample estimates for comparison. 
Column (4) reports p-values from Wald tests of coefficient differences between COVID and 
pre-COVID periods. Driscoll--Kraay standard errors (bandwidth = 3) in parentheses. 
$^{*}$ p $<$ 0.10, $^{**}$ p $<$ 0.05, $^{***}$ p $<$ 0.01.
\end{minipage}
\end{tablenotes}
\end{threeparttable}
\end{table}


==> table3_price_robustness_copy.tex <==
\begin{table}[p]
\centering
\caption{Robustness to Alternative Price Measures: Pre-COVID Period (2010--2019)}
\label{tab:price_robustness}
\begin{threeparttable}
\begin{adjustbox}{width=\textwidth}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{@{}lcccccc@{}}
\toprule
& \multicolumn{6}{c}{Price Measurement} \\
\cmidrule(lr){2-7}
& \multicolumn{2}{c}{Income-Relative} & \multicolumn{2}{c}{PPP-Adjusted} & \multicolumn{2}{c}{Nominal USD} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& EU & EaP & EU & EaP & EU & EaP \\
& (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\textbf{Price Elasticity} \\
Log(Price) & $-0.12^{**}$ & -- & $-0.14^{**}$ & -- & $-0.09^{*}$ & -- \\
& (0.05) & & (0.05) & & (0.05) & \\
\\
Log(Price) $\times$ EaP & -- & $-0.49^{***}$ & -- & $-0.50^{***}$ & -- & $-0.48^{***}$ \\
& & (0.09) & & (0.10) & & (0.10) \\
\\
\textit{Implied EaP elasticity} & -- & $-0.61^{***}$ & -- & $-0.64^{***}$ & -- & $-0.57^{***}$ \\
& & (0.08) & & (0.09) & & (0.09) \\
\midrule
\textbf{Model Statistics} \\
Full controls & Yes & Yes & Yes & Yes & Yes & Yes \\
Country FE & Yes & Yes & Yes & Yes & Yes & Yes \\
Year FE & Yes & Yes & Yes & Yes & Yes & Yes \\
Observations & 297 & 297 & 297 & 297 & 297 & 297 \\
R-squared & 0.92 & 0.92 & 0.91 & 0.91 & 0.90 & 0.90 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\begin{tablenotes}[flushleft]
\scriptsize
\begin{minipage}{\textwidth}
\item \textit{Notes:} Dependent variable is log of fixed broadband subscriptions per 100 inhabitants. 
Columns (1)--(2) use income-relative prices (price as \% of GNI per capita) as baseline. 
Columns (3)--(4) use PPP-adjusted prices in international dollars. Columns (5)--(6) use nominal 
USD prices. All specifications include full controls: log GDP per capita, urban population \%, 
tertiary enrollment \%, regulatory quality, log secure servers, R\&D \% GDP, log population 
density, and age dependency ratio. EaP is a dummy for Eastern Partnership countries 
(Armenia, Azerbaijan, Belarus, Georgia, Moldova, Ukraine). Driscoll--Kraay standard errors 
(bandwidth = 3) in parentheses. $^{*}$ p $<$ 0.10, $^{**}$ p $<$ 0.05, $^{***}$ p $<$ 0.01.
\end{minipage}
\end{tablenotes}
\end{threeparttable}
\end{table}


==> table4_placebo_copy.tex <==
\begin{table}[p]
\centering
\caption{Placebo Test: Pre-COVID Trends (2010--2019)}
\label{tab:placebo}
\begin{threeparttable}
\begin{adjustbox}{max width=\textwidth}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.85}
\begin{tabular}{@{}lccc@{}}
\toprule
& \multicolumn{3}{c}{Dependent Variable: Log(Subs. per 100)} \\
\cmidrule(lr){2-4}
& (1) & (2) & (3) \\
& Full Sample & Early & Late \\
& 2010--19 & 2010--14 & 2015--19 \\
\midrule
\textbf{Panel A: EU Countries} \\
Log(Price) & $-0.11^{*}$ & $-0.13^{*}$ & $-0.04$ \\
& (0.06) & (0.07) & (0.07) \\
Log(Price) $\times$ Late & $+0.08$ & -- & -- \\
& (0.08) & & \\
\textit{Implied late elasticity} & $-0.03$ & -- & $-0.04$ \\
& (0.09) & & (0.07) \\
\midrule
\textbf{Panel B: EaP Countries} \\
Log(Price) $\times$ EaP & $-0.48^{***}$ & $-0.52^{***}$ & $-0.25^{**}$ \\
& (0.10) & (0.11) & (0.11) \\
Log(Price) $\times$ EaP $\times$ Late & $+0.27^{**}$ & -- & -- \\
& (0.13) & & \\
\textit{Implied early EaP elasticity} & $-0.59^{***}$ & $-0.65^{***}$ & -- \\
& (0.09) & (0.10) & \\
\textit{Implied late EaP elasticity} & $-0.32^{**}$ & -- & $-0.29^{**}$ \\
& (0.12) & & (0.11) \\
\midrule
\textbf{Panel C: Change in Elasticity} \\
$\Delta\varepsilon_{EU}$ (Late - Early) & $+0.08$ & -- & -- \\
& (0.08) & & \\
p-value & 0.31 & -- & -- \\
$\Delta\varepsilon_{EaP}$ (Late - Early) & $+0.27^{**}$ & -- & -- \\
& (0.13) & & \\
p-value & 0.045 & -- & -- \\
\midrule
\textbf{Panel D: Model Statistics} \\
Full controls & Yes & Yes & Yes \\
Country FE & Yes & Yes & Yes \\
Year FE & Yes & Yes & Yes \\
Observations & 297 & 165 & 165 \\
Countries & 33 & 33 & 33 \\
R-squared & 0.92 & 0.88 & 0.94 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{4pt}
\begin{tablenotes}[para,flushleft]
\scriptsize
\begin{minipage}{\textwidth}
\item \textit{Notes:} Dependent variable: log fixed broadband subscriptions per 100. Price: \% of GNI per capita. ``Late'' is a placebo indicator for 2015--2019. EaP denotes Eastern Partnership countries. Column (1) estimates the full placebo interaction on 2010--2019; Columns (2)--(3) report subsamples for 2010--2014 (early) and 2015--2019 (late). Controls in all models: log GDP per capita, urbanization (\%), tertiary enrollment (\%), regulatory quality, log secure servers, R\&D (\% GDP), log population density, and age dependency ratio. The positive EaP interaction ($+0.27$, p = 0.045) suggests elasticity was already declining pre-COVID. Driscoll--Kraay SEs (bandwidth = 3) in parentheses. $^{*}$ p $<$ 0.10, $^{**}$ p $<$ 0.05, $^{***}$ p $<$ 0.01.
\end{minipage}
\end{tablenotes}
\end{threeparttable}
\end{table}

